Joint Geometric and Topological Analysis of Hierarchical Datasets

In a world abundant with diverse data arising from complex acquisition techniques, there is a growing need for new data analysis methods. In this paper we focus on high-dimensional data that are organized into several hierarchical datasets. We assume that each dataset consists of complex samples, and every sample has a distinct irregular structure modeled by a graph. The main novelty in this work lies in the combination of two complementing powerful data-analytic approaches: topological data analysis (TDA) and geometric manifold learning. Geometry primarily contains local information, while topology inherently provides global descriptors. Based on this combination, we present a method for building an informative representation of hierarchical datasets. At the finer (sample) level, we devise a new metric between samples based on manifold learning that facilitates quantitative structural analysis. At the coarser (dataset) level, we employ TDA to extract qualitative structural information from the datasets. We showcase the applicability and advantages of our method on simulated data and on a corpus of hyper-spectral images. We show that an ensemble of hyper-spectral images exhibits a hierarchical structure that fits well the considered setting. In addition, we show that our new method gives rise to superior classification results compared to state-of-the-art methods.

==> Sections/Bibliography.tex <==
% 1
\bibitem{shnitzer2019recovering}
Shnitzer T., Ben-Chen M., Guibas L.,  Talmon R,.  Wu H,.:
Recovering Hidden Components in Multimodal Data with Composite Diffusion Operators.
SIAM Journal on Mathematics of Data Science.
\textbf{1}(3), 588-616, (2019)
% 2
\bibitem{diffusion_maps}
Coifman R. R., Lafon S.: Diffusion maps.
Applied and Computational Harmonic Analysis,
\textbf{21}(1), 5-30, (2006),
% 3
\bibitem{Alternating_diffusion}
Lederman R. R., Talmon R.:
Learning the geometry of common latent variables using alternating-diffusion.
Applied and Computational Harmonic Analysis,
\textbf{44}(3), 509 - 536 (2018)
% 4
\bibitem{Icones-HSI-data}
Ben-Ahmed O., Urruty T., Noel R., Fernandez-Maloigne C.:
Toward Content-Based Hyperspectral Remote Sensing Image Retrieva (CB-HRSIR): A Preliminary Study Based on Spectral Sensitivity Functions.
Remote. Sens. \textbf{11}(5), 600 - 615 (2019)
% 5
\bibitem{AVIRIS}
NASA Jet Propulsion Laboratory's Airborne Visible InfraRed Imaging Spectrometer (AVIRIS), \url{https://aviris.jpl.nasa.gov/}. Last accessed 1 Mar 2021.
% 6
\bibitem{TSNE}
Van-der-Maaten L., Hinton G.: Visualizing Data using t-SNE.
Journal of Machine Learning Research,
\textbf{9}(86), 2579-2605 (2008)
% 7
\bibitem{SVM}
Cortes C., Vapnik V.: Support-Vector Networks. Mach. Learn., \textbf{20}(3), 273–297 (1995)
% 8
\bibitem{Wasserstein}
Mileyko Y., Mukherjee S., Harer J.: Probability measures on the space of persistence diagrams.
Inverse Problems \textbf{27}(12), 124007 (2011)
% 9
\bibitem{ISOMAP}
Tenenbaum J.B., Vin de S., Langford J.C.: A Global Geometric Framework for Nonlinear Dimensionality Reduction.
Science \textbf{290}(5500), 2319-2323 (2000).
% 10
\bibitem{LLE}
Roweis  S.T., Lawrence K.S.: Nonlinear Dimensionality Reduction by Locally Linear Embedding
Science \textbf{290}(5500), 2323-2326 (2000).
% 11
\bibitem{belkin2003laplacian}
Belkin M., Niyogi P.: Laplacian Eigenmaps for Dimensionality Reduction and Data Representation.
Neural Computation. \textbf{15}(6), 1373-1396 (2003).
% 12
\bibitem{TDA_1}
Carlsson G.: Topology and data.
Bulletin of the American Mathematical Society, \textbf{46}(2), 255 – 308 (2009).
% 13
\bibitem{TDA_2}
Ghrist R.: Barcodes: The persistent topology of data. 
Bulletin of the American Mathematical Society, \textbf{45}(01), 61 – 76 (2007).
% 14
\bibitem{TDA_3}
Wasserman L.: Topological data analysis. 
Annual Review of Statistics and Its Application, \textbf{5}(1), 501 – 532 (2018).
% 15
\bibitem{singer2015spectral}
Singer A.,  Wu H.-T.: Spectral convergence of the connection Laplacian from random samples.
Information and Inference, 6, 58-123 (2016).
% 16
\bibitem{Froyland_2015}
Froyland G.: Dynamic isoperimetry and the geometry of Lagrangian coherent structures.
Nonlinearity, \textbf{28}(10), 3587-3622 (2015).
% 17
\bibitem{Froyland2020}
Froyland G., Kwok G.:  A Dynamic Laplacian for Identifying Lagrangian Coherent Structures on Weighted Riemannian Manifolds.
Journal of Nonlinear Science, \textbf{5}(30), 1-83 (2017).
% 18
\bibitem{Presistent_Homology_1}
Edelsbrunner H., Letscher D., Zomorodian A.: Topological persistence and simplification.
Discrete \& Computational Geometry, \textbf{28}(4), 511–533 (2002)
% 19
\bibitem{Presistent_Homology_2}
Edelsbrunner H., Harer J.: Persistent homology — a survey.
Discrete \& Computational Geometry, 453, 257-282 (2008).
% 20
\bibitem{Presistent_Homology_3}
Edelsbrunner H., Morozov. D.: Persistent homology: Theory and practice. 
In: European Congress of Mathematics. pp 31–-50.
European Mathematical Society Publishing House, Kraków, (2014).
% 21
\bibitem{Presistent_Homology_4}
Hatcher A.: Algebraic topology. 1st edn. Cambridge University Press, Cambridge, 2002.
% 22 
\bibitem{Presistent_Homology_5}
Zomorodian A., Carlsson G.: Computing persistent homology.
Discrete \& Computational Geometry, \textbf{33}(2). 249–274 (2004).
% 23
\bibitem{ADlederman}
Lederman R.R., Talmon R.: Learning the geometry of common latent variables using alternating-diffusion.
Applied and Computational Harmonic Analysis, \textbf{44}(3). 509-536 (2018).
% 24
\bibitem{IMC}
Giesen, C., Wang, H., Schapiro, D. et al.: Highly multiplexed imaging of tumor tissues with subcellular resolution by mass cytometry.
Nature Methods \textbf{4}(11), 417–422 (2014). 
% 25
\bibitem{GeneExp}
Edgar R., Domrachev M., Lash E.A.: Gene Expression Omnibus: NCBI gene expression and hybridization array data repository.
Nucleic Acids Research, \textbf{30}(1), 207–210 (2002).
% 26
\bibitem{ProteinData}
Cannataro M., Pietro H.G., Pierangelo V.:,
Protein-to-Protein Interactions: Technologies, Databases, and Algorithms.
ACM Computing Survey, \textbf{43}(1), 1-36 (2010).
% 27
\bibitem{Networks}
Leskovec J., Krevl A.: SNAP Datasets: Stanford Large Network Dataset Collection.
\url{http://snap.stanford.edu/data}, Last accessed 14 Mar 2021.
% 28
\bibitem{MRI}
LaMontagne J.P., Benzinger T., et. al.:
OASIS-3: Longitudinal Neuroimaging, Clinical, and Cognitive Dataset for Normal Aging and Alzheimer Disease.
medRxiv, Cold Spring Harbor Laboratory Press (2019).
% 29
\bibitem{Wasserstein_2}
Cohen-Steiner D., Edelsbrunner H.,  Harer J.: Stability of persistence diagrams.
Discrete \& Computational Geometry, \textbf{37}(1), 103–120 (2007).
% 30
\bibitem{ML_TDA}
Seng-Pun C., Xia K., Xian Lee S.: Persistent-homology-based machine learning and its applications – a survey.
SSRN Electronic Journal, 2018. 
% 31
\bibitem{image_TDA_1}
Lawson P., Sholl B.A., Brown J.Q., Fasy T.B., Wenk C.: Persistent homology for the quantitative evaluation of architectural features in prostate cancer histology.
Scientific Reports, \textbf{9}(1), 1-15 (2019).
% 32
\bibitem{image_TDA_2}
Qaiser T, Tsang Y.W., Taniyama D., Sakamoto N., Nakane K, Epstein D.,  Rajpoot N.: Fast and accurate tumor segmentation of histology images using persistent homology and deep convolutional features.
Medical Image Analysis, 55: 1–14 (2019).
% 33
\bibitem{shape_TDA_1}
Li C., Ovsjanikov M., Chazal F.: Persistence-based structural recognition.
In 2014 IEEE Conference on Computer Vision and Pattern Recognition. IEEE, Columbus, pp. 2003-2010,(2014). doi: 10.1109/CVPR.2014.257.
% 34
\bibitem{shape_TDA_2}
Skraba P., Ovsjanikov M., Chazal F., Guibas L.: Persistence-based segmentation of deformable shapes. 
In 2010 IEEE Computer Society Conference on Computer Vision
and Pattern Recognition - Workshops. San Francisco,  USA, 2010, pp. 45-52, doi: 10.1109/CVPRW.2010.5543285.
% 35
\bibitem{shape_TDA_3}
Crawford L., Monod A., Chen X.A., Mukherjee S., Rabadán R.: Predicting clinical outcomes in glioblastoma: An application of topological and functional data analysis.
Journal of the American Statistical Association, \textbf{115} (531). 1139–1150 (2020).
% 36
\bibitem{DL_TDA_1}
Hofer C., Kwitt R., Niethammer M., Uhl A.: Deep learning with topological signatures. In Advances in Neural Information Processing Systems, \textbf{30}. Curran Associates, Inc. (2017).
% 37
\bibitem{DL_TDA_2}
Hu X., Li F., Samaras D., Chen C.. Topology-preserving deep image
segmentation. In Advances in Neural Information Processing Systems,  \textbf{32}, 2019.
% 38
\bibitem{DL_TDA_3}
Gabrielsson B.R., Nelson J.B., Dwaraknath A., Skraba P.: A topology layer for machine learning. In Proceedings of the Twenty Third International Conference on Artificial Intelligence and Statistics,  108, pp. 1553--1563 (2020).
% 39
\bibitem{DL_TDA_4}
Naitzat G., Zhitnikov A., Lim L.H.: Topology of deep neural networks.
Journal of Machine Learning Research, \textbf{21}(184), 1–40 (2020).
% 40
\bibitem{dynamical_systems_1}
Nadler B., Lafon S., Coifman R.R., Kevrekidis G.I: Diffusion maps, spectral clustering and reaction coordinates of dynamical systems.
Applied and Computational Harmonic Analysis, \textbf{21}(1), 113-127 (2006).
% 41
\bibitem{dynamical_systems_2}
Froyland G.:Dynamic isoperimetry and the geometry of Lagrangian coherent structures.
Nonlinearity, \textbf{28}(10), 3587-3622 (2015).
% 42
\bibitem{multi_modal_1}
Lahat D., Adali T., Jutten C.: Multimodal Data Fusion: An Overview of Methods, Challenges, and Prospects.
In: Proceedings of the IEEE, \textbf{103}(9),  1449--1477 (2015).
% 43
\bibitem{multi_view}
Davenport M.A., Hegde C., Duarte M.F., Baraniuk R.G.: Joint manifolds for data fusion. 
IEEE Transactions on Image Processing, \textbf{19}(10), 2580-2594 (2010).
% 44
\bibitem{UMAP}
McInnes L., Healy J.: UMAP: Uniform Manifold Approximation and Projection for Dimension Reduction.
ArXiv e-prints, (2018).
% 45 
\bibitem{HSI_tech}
Chein-I C.: Hyperspectral imaging: techniques for spectral detection and classification. 
Springer Science \& Business Media, (2003).

% TODO: use bibtex. copied from proposal

\bibitem{Tenenbaum2000}
J.~B. Tenenbaum, V.~de~Silva, and J.~C. Langford,
\newblock ``A global geometric framework for nonlinear dimensionality
  reduction,''
\newblock {\em Science}, vol. 260, pp. 2319--2323, 2000.

\bibitem{Roweis2000}
S.~T. Roweis and L.~K. Saul,
\newblock ``Nonlinear dimensionality reduction by locally linear embedding,''
\newblock {\em Science}, vol. 260, pp. 2323--2326, 2000.

\bibitem{Belkin2003}
M.~Belkin and P.~Niyogi,
\newblock ``Laplacian eigenmaps for dimensionality reduction and data
  representation,''
\newblock {\em Neural Comput.}, vol. 15, pp. 1373--1396, 2003.

\bibitem{Coifman2006}
R.~Coifman and S.~Lafon,
\newblock ``Diffusion maps,''
\newblock {\em Appl. Comput. Harmon. Anal.}, vol. 21, pp. 5--30, Jul. 2006.

\bibitem{carlsson_topology_2009}
Gunnar Carlsson,
\newblock ``Topology and data,''
\newblock {\em Bulletin of the American Mathematical Society}, vol. 46, no. 2,
  pp. 255--308, 2009.

\bibitem{ghrist_barcodes:_2008}
Robert Ghrist,
\newblock ``Barcodes: the persistent topology of data,''
\newblock {\em Bulletin of the American Mathematical Society}, vol. 45, no. 1,
  pp. 61--75, 2008.

\bibitem{wasserman_topological_2016}
Larry Wasserman,
\newblock ``Topological {Data} {Analysis},''
\newblock {\em arXiv:1609.08227 [stat]}, Sept. 2016,
\newblock arXiv: 1609.08227.

\bibitem{chazal2017introduction}
Fr{\'e}d{\'e}ric Chazal and Bertrand Michel,
\newblock ``An introduction to topological data analysis: fundamental and
  practical aspects for data scientists,''
\newblock {\em arXiv preprint arXiv:1710.04019}, 2017.

\bibitem{adler_modeling_2017}
Robert~J. Adler, Sarit Agami, and Pratyush Pranav,
\newblock ``Modeling and replicating statistical topology and evidence for
  {CMB} nonhomogeneity,''
\newblock {\em Proceedings of the National Academy of Sciences}, vol. 114, no.
  45, pp. 11878--11883, Nov. 2017.

\bibitem{nicolau_topology_2011}
Monica Nicolau, Arnold~J Levine, and Gunnar Carlsson,
\newblock ``Topology {Based} {Data} {Analysis} {Identifies} a {Subgroup} of
  {Breast} {Cancers} with a {Unique} {Mutational} {Profile} and {Excellent}
  {Survival},''
\newblock {\em Proceedings of the National Academy of Sciences}, Apr. 2011.

\bibitem{hiraoka_hierarchical_2016}
Yasuaki Hiraoka, Takenobu Nakamura, Akihiko Hirata, Emerson~G. Escolar, Kaname
  Matsue, and Yasumasa Nishiura,
\newblock ``Hierarchical structures of amorphous solids characterized by
  persistent homology,''
\newblock {\em Proceedings of the National Academy of Sciences}, vol. 113, no.
  26, pp. 7035--7040, June 2016.

\bibitem{chan_topology_2013}
Joseph~Minhow Chan, Gunnar Carlsson, and Raul Rabadan,
\newblock ``Topology of viral evolution,''
\newblock {\em Proceedings of the National Academy of Sciences}, vol. 110, no.
  46, pp. 18566--18571, Nov. 2013.

\bibitem{taylor_topological_2015}
Dane Taylor, Florian Klimm, Heather~A. Harrington, Miroslav Kram{\'a}r,
  Konstantin Mischaikow, Mason~A. Porter, and Peter~J. Mucha,
\newblock ``Topological data analysis of contagion maps for examining spreading
  processes on networks,''
\newblock {\em Nature communications}, vol. 6, 2015.

\bibitem{bendich_persistent_2016}
Paul Bendich, James~Stephen Marron, Ezra Miller, Alex Pieloch, and Sean
  Skwerer,
\newblock ``Persistent homology analysis of brain artery trees,''
\newblock {\em The Annals of Applied Statistics}, vol. 10, no. 1, pp. 198--218,
  2016.

\bibitem{coifman2005geometric}
Ronald~R Coifman, Stephane Lafon, Ann~B Lee, Mauro Maggioni, Boaz Nadler,
  Frederick Warner, and Steven~W Zucker,
\newblock ``Geometric diffusions as a tool for harmonic analysis and structure
  definition of data: Diffusion maps,''
\newblock {\em Proceedings of the National Academy of Sciences of the United
  States of America}, vol. 102, no. 21, pp. 7426--7431, 2005.

\bibitem{coifman2008diffusion}
R.R. Coifman, I.G. Kevrekidis, S.~Lafon, M.~Maggioni, and B.~Nadler,
\newblock ``Diffusion maps, reduction coordinates, and low dimensional
  representation of stochastic systems,''
\newblock {\em Multiscale Modeling \& Simulation}, vol. 7, no. 2, pp. 842--864,
  2008.

\bibitem{TalmonPNAS}
R.~Talmon and R.R. Coifman,
\newblock ``Empirical intrinsic geometry for nonlinear modeling and time series
  filtering,''
\newblock {\em Proc. Nat. Acad. Sci.}, vol. 110, no. 31, pp. 12535--12540,
  2013.

\bibitem{dabaghian_topological_2012}
Yu~Dabaghian, Facundo M{\'e}moli, L.~Frank, and Gunnar Carlsson,
\newblock ``A topological paradigm for hippocampal spatial map formation using
  persistent homology,''
\newblock {\em PLoS computational biology}, vol. 8, no. 8, pp. e1002581, 2012.

\bibitem{giusti_clique_2015}
Chad Giusti, Eva Pastalkova, Carina Curto, and Vladimir Itskov,
\newblock ``Clique topology reveals intrinsic geometric structure in neural
  correlations,''
\newblock {\em Proceedings of the National Academy of Sciences}, vol. 112, no.
  44, pp. 13455--13460, 2015.

\bibitem{petri_homological_2014}
Giovanni Petri, Paul Expert, Federico Turkheimer, Robin Carhart-Harris, David
  Nutt, Peter~J. Hellyer, and Francesco Vaccarino,
\newblock ``Homological scaffolds of brain functional networks,''
\newblock {\em Journal of The Royal Society Interface}, vol. 11, no. 101, pp.
  20140873, 2014.

\bibitem{lum_extracting_2013}
P.~Y. Lum, G.~Singh, A.~Lehman, T.~Ishkanov, Mikael Vejdemo-Johansson,
  M.~Alagappan, J.~Carlsson, and G.~Carlsson,
\newblock ``Extracting insights from the shape of complex data using
  topology,''
\newblock {\em Scientific reports}, vol. 3, 2013.

\bibitem{singh_topological_2008}
Gurjeet Singh, Facundo Memoli, Tigran Ishkhanov, Guillermo Sapiro, Gunnar
  Carlsson, and Dario~L. Ringach,
\newblock ``Topological analysis of population activity in visual cortex,''
\newblock {\em Journal of vision}, vol. 8, no. 8, pp. 11, 2008.

\bibitem{shuman2013emerging}
D.~I Shuman, S.~K. Narang, P.~Frossard, A.~Ortega, and P.~Vandergheynst,
\newblock ``The emerging field of signal processing on graphs: Extending
  high-dimensional data analysis to networks and other irregular domains,''
\newblock {\em IEEE Signal Processing Magazine}, vol. 30, no. 3, pp. 83--98,
  2013.

\bibitem{zomorodian_topological_2007}
Afra Zomorodian,
\newblock ``Topological data analysis,''
\newblock {\em Advances in Applied and Computational Topology}, vol. 70, pp.
  1--39, 2007.

\bibitem{lee2011multiscale}
Jason~D Lee and Mauro Maggioni,
\newblock ``Multiscale analysis of time series of graphs,''
\newblock in {\em International Conference on Sampling Theory and Applications
  (SampTA)}, 2011.

\bibitem{rabin2010data}
Neta Rabin,
\newblock {\em Data mining in dynamically evolving systems via diffusion
  methodologies},
\newblock Ph.D. thesis, Tel Aviv University, 2010.

\bibitem{coifman2014diffusion}
Ronald~R Coifman and Matthew~J Hirn,
\newblock ``Diffusion maps for changing data,''
\newblock {\em Applied and computational harmonic analysis}, vol. 36, no. 1,
  pp. 79--107, 2014.

\bibitem{marshall2017time}
Nicholas~F Marshall and Matthew~J Hirn,
\newblock ``Time coupled diffusion maps,''
\newblock {\em Applied and Computational Harmonic Analysis}, 2017.

\bibitem{pennec2006riemannian}
Xavier Pennec, Pierre Fillard, and Nicholas Ayache,
\newblock ``A riemannian framework for tensor computing,''
\newblock {\em International Journal of computer vision}, vol. 66, no. 1, pp.
  41--66, 2006.

\bibitem{lederman2015learning}
Roy~R Lederman and Ronen Talmon,
\newblock ``Learning the geometry of common latent variables using
  alternating-diffusion,''
\newblock {\em Applied and Computational Harmonic Analysis}, 2015.

\bibitem{talmon2017latent}
Ronen Talmon and Hau-tieng Wu,
\newblock ``Latent common manifold learning with alternating diffusion:
  analysis and applications,''
\newblock {\em Applied and Computational Harmonic Analysis}, 2017.



==> Sections/Code.tex <==

\begin{itemize}
    \item The Python code generating the results presented in Sections 5 and 6 is available in this additional material. To maintain author anonymity, the code will be uploaded to GitHub and made publicly available only upon acceptance of the paper.
    % \href{https://github.com/LiorAl/geometric-topological}{here}. 
    See README.md file for detailed instructions. %\footnote{\url{https://github.com/LiorAl/geometric-topological}}. 
    The code makes use of a TDA software package from \cite{maria2014gudhi}.
    \item The HSI database is publicly available and can be downloaded from \href{http://xlim-sic.labo.univ-poitiers.fr/datasets/ICONES-HSI}{here}.
    %\footnote{\url{http://xlim-sic.labo.univ-poitiers.fr/datasets/ICONES-HSI}}.
\end{itemize}

